Do accretion-powered stellar winds help spin down T Tauri stars?

How T Tauri stars remain slowly rotating while still accreting material is a long-standing puzzle. Current models suggest that these stars may lose angular momentum through magnetospheric ejections of disk material (MEs) and accretion-powered stellar winds (APSWs). The individual contribution of each mechanism to the stellar spin evolution, however, is unclear. We explore how these two scenarios could be distinguished by applying stellar spin models to near-term observations. We produce synthetic stellar populations of accreting Class II stars with spreads in the parameters governing the spin-down processes and find that an APSW strongly affects the ratio of the disk truncation radius to the corotation radius, $\mathcal{R} = R_\mathrm{t}/R_\mathrm{co}$. The ME and APSW scenarios are distinguished to high confidence when at least $N_\mathrm{crit}\gtrsim 250$ stars have values measured for $\mathcal{R}$. Newly developed lightcurve analysis methods enable measuring $\mathcal{R}$ for enough stars to distinguish the spin-down scenarios in the course of upcoming observing campaigns.

==> resources/old_sections/acknowledgments.tex <==
\begin{acknowledgements}

EG was supported by NASA Award  80NSSC19K0587 (Astrophysics Data Analysis Program) and NSF Award 2106927
(Astronomy \& Astrophysics Research Program) as a Gauss Professor at the University of G\"{o}ttingen by the Nieders\"{a}chsische Akaemie der Wissenschaften.
 
\end{acknowledgements}

==> resources/old_sections/discussion.tex <==
% ------------------------------------------------------------------

\section{Discussion and Conclusion}
\label{sec:discussion}



In this work, we have constructed a stellar spin population model focusing on the differences between the no-wind and wind scenarios.
In particular, the value of $R_\mathrm{t}/R_\mathrm{co}$ is affected by the presence of an APSW.
Now, we discuss the sensitivity of our results to different conditions, the availability of observations to test our predictions, and the main limitation of our model.


\subsection{Sensitivity test}\label{sec:sens}


In the SPM, we randomly choose the magnetic field strength and the stellar rotation period from the expected variation since the actual distributions of these parameters are poorly constrained.  Now, we choose these parameters differently and study the respective sensitivity of our results. 
First, we change the distribution of $B_\star$.
While the range is still between 0.1 and 2.0~kG, the distribution is centered at 1.5~kG with a deviation of 0.3~kG, shifting the magnetic field strengths to higher values.
As a result, the theoretical difference between the wind and no-wind scenarios decreases (see \fig{fig:theo_age}), and the expected variation increases (see \fig{fig:delta}).  This is reflected by an increase in $N_\mathrm{crit}$ by 30\%.  Next, we adapt the torque variation due to short-term variability (see \sref{sec:uncert}).   The torque can still vary between $2\Delta_\mathrm{spin~up}$ and $2\Delta_\mathrm{spin~down}$ but it is chosen from a normal distribution located at the center of $\Delta_\mathrm{spin~up}$ and $\Delta_\mathrm{spin~down}$ with a deviation of the distance between the center $\Delta_\mathrm{spin~up}$.  As a result, the rotation periods are located closer to the equilibrium state, and the value of $N_\mathrm{crit}$ decreases by 18\%.


In this work, we have restricted the wind parameter $W$ to two values, 0\% and 1\%.
It is, however, likely that the values of $W$ are distributed along a certain range.
We want to discuss how our results would be affected if $W$ is distributed uniformly between 0\% and 2\%.
Although the variation is mostly unaffected by the value of $W$ (see \sref{sec:uncert}), the equilibrium value of $\mathcal{R}$ would change (see \sref{sec:equi_theo}).
For lower values of $W$ the equilibrium states of the no-wind and wind scenarios are located closer together resulting in more similar distributions and an increase in $N_\mathrm{crit}$.
Similarly, for higher values of $W$, $N_\mathrm{crit}$ decreases.
As a result, using the aforementioned uniform distribution of $W$ between 0\% and 2\%, the mean values of the distributions should remain approximately constant while the scatter increases.
Thus, $N_\mathrm{crit}$ would also increase but should remain in the same order of magnitude.
We note that this estimation can change based on the assumed distribution of $W$.





\subsection{Availability of observations}\label{sec:obs}

Several studies have collected an impressive number of stellar parameters in recent years, including the stellar mass, radius, rotation period, and accretion rate \citep[e.g.,][]{Betti2023, Smith2023}.
On the other hand, the large-scale magnetic field strength and the position of the truncation radius are poorly constrained by observations.
Currently, there are a few dozen observations of magnetic field strengths of accreting stars \citep[e.g.,][]{Johnstone14, Reiners22} and about as many $R_\mathrm{t}$ estimates derived from constraining the size of the Br$\gamma$ emitting region around young stars with interferometric observations \citep{Eisner2014,Gravity2023}.
These numbers are not sufficient to test the SPM adequately.

% now comes the new technique
However, the 1-dimensional model of time-dependent accretion in young stars by \citet{Robinson2021} has recently enabled the development of the first prescription that directly links the light curve morphology and color variability of accreting young stars to the underlying magnetospheric accretion structure. The theoretical underpinning of this prescription is the following: the kinetic energy of the accretion flow deposited onto the star depends on the distance it traveled from its starting point $R_\mathrm{t}$. 
This dependence is reflected in the emission spectrum of the resulting accretion shock, which can be probed observationally by measuring the color of the ultraviolet (UV) excess.% emission induced by the accretion shock and its time variability over stellar rotation timescales. 
A pilot observational program to validate this prescription is presented in Venuti et al. (2025, in prep.), who employ simultaneous monitoring data of accreting young stars at near-UV and optical wavelengths to populate the stellar loci on color-magnitude diagrams and fit them with the \citet{Robinson2021} grid of predicted color traces to identify the best-fitting magnetospheric parameters.
Derived independently of other observational parameters, the value of $R_\mathrm{t}$ in combination with $\Dot{M}_\star$ and $P_\star$ can also provide estimates of $B_\star$ (see \equo{eq:Rt}).
Thus, the large-scale application of the technique described in Venuti et al. (2025, in prep.) could provide a significant number of $R_\mathrm{t}$ and $B_\star$ measurements, thereby allowing valuable insights into stellar spin-down mechanisms.




\subsection{Accuracy of the stellar spin model}\label{sec:limits}


The main limitation of the SPM lies in the spin model itself.
In their study, \cite{Ireland2022} utilize 2.5-dimensional simulations of the star-disk interaction region.
Based on these simulations, with simulation times over several dynamical timescales ($\lesssim 50~\mathrm{P_\star}$), relations for the torque acting on the star are extracted \citep[see also][]{Pantolmos20} and extrapolated over a large parameter space and the lifetime of PPDs \citep[e.g.,][]{Ireland21}.
While producing correct qualitative correlations, the absolute results of the spin model are subjected to uncertainties.


One example is the stellar rotation periods of the SPM.
While the range of observed periods between $\sim 1$ and $\sim 10$~days are reproduced, the maximum is located at 1-3~days. 
This is faster compared to the observed maximum at 3-4~days \citep[e.g.,][]{Smith2023}.
When comparing different stellar spin models, we find that the parameter $K_\mathrm{t,1}$ used in \cite{Ireland2022} is smaller in the SPM by a factor of 0.67, compared to the values presented in \cite{Gallet19} and \cite{Pantolmos20}.
As a result, for a given value of $\mathcal{R}$, the truncation radius and the corotation radius are smaller.
A smaller corotation radius is connected to faster rotation and the periods calculated by the SPM are up to a factor of 0.55 faster compared to the other models \citep[][]{Gallet19, Pantolmos20}. 
This could explain the faster rotation in the SPM compared to observations.
We note that this quick comparison only accounts for the different parameters determining $R_\mathrm{t}$.
A more detailed study is required to identify the differences between specific spin models.
Another aspect that varies between different spin models is the amount of angular momentum added to the star due to accretion.
Magnetic torques and outflows, such as MEs, can remove AM of the disk and at $R_\mathrm{t}$, the disk rotates at velocities smaller than Keplerian \citep[e.g.,][]{Gallet19}.
The closer the disk rotates to the Keplerian value, the more AM it carries, and the greater the stellar spin-up tendency.
In different models, the disks rotate between 0.4 \citep[][]{Gallet19} and 0.9 \citep[][]{Ireland2022} of the Keplerian value.

Nevertheless, the SPM presented in this work should still be able to produce qualitative results and should be treated as a proof-of-concept study.
We highlight the sensitivity of the value $\mathcal{R}$ in the presence of an APSW.
With sufficient observations, different stellar spin-down mechanisms should be distinguishable, knowing that different spin models could lead to different distributions.
Thus, a careful evaluation of available stellar spin models is recommended when comparing the SPM to future observations.












\subsection{Concluding remarks}

According to recent spin evolution models, an accreting star can spin down due to magnetospheric ejections or an accretion-powered stellar wind.
The dominant spin-down process, however, is still unclear.
The primary purpose of this letter is to sketch a method that can identify what spins down a young star based on observations.
A key difference between the spin-down mechanisms manifests itself in the value of $\mathcal{R} = R_\mathrm{t}/R_\mathrm{co}$.
As the stellar spin evolution model tends to find an equilibrium (or zero-torque) state, removing angular momentum by an APSW will reduce $\mathcal{R}$ compared to a no-wind scenario.
Within our SPM, approximately $N_\mathrm{crit}\gtrsim 200-250$~stars (with simultaneous measurements of $\mathcal{R}$, $P_\star$, and $\Mdot$) are required to differentiate between the no-wind and wind scenarios at a high ($3\sigma$) confidence level.
The stellar ages for this comparison should be between $\gtrsim 2$ and $\sim 5$~Myr.
Unfortunately, testing our model on observations poses a problem due to the lack of necessary measurements of $B_\star$ or $R_\mathrm{t}$.
A novel observational technique can provide the required number of observations for $R_\mathrm{t}$, allowing detailed tests of our SPM during future campaigns.












==> resources/old_sections/header.tex <==
%
\titlerunning{Tests of angular momentum regulation in T~Tauri stars}
%Observing what spins down a low-mass accreting protostar
\authorrunning{L.~Gehrig \& ...}
\title{Tests of angular momentum regulation in T~Tauri stars} 
%
% \subtitle{I. The embedded phase}
%
\author{
 Lukas~Gehrig\inst{1}, Eric Gaidos\inst{1,2}, Laura Venuti\inst{3,4} and Ann Marie Cody\inst{3}
}
%
\institute{
 Department of Astrophysics, University of Vienna,
 Türkenschanzstrasse 17, A-1180 Vienna, Austria
 \and
 Department of Earth Sciences, University of Hawai'i at M\={a}noa, Honolulu, Hawai'i 96822 USA
 \and
 SETI Institute, 339 Bernardo Ave., Suite 200, Mountain View, CA 94043, USA
\and
Visiting Fellow, School of Physics, UNSW Science, Kensington, NSW 2052, Australia
}
%\today
\date{Received ....; accepted ....}

\abstract
{
It is still unclear how T~Tauri stars are prevented from spinning up. 
Current models suggest stellar angular momentum is removed either due to magnetospheric ejections (MEs) or by launching an accretion-powered stellar wind (APSW).
% }
% {
% We explore the possibility of differentiating between these spin-down scenarios by comparing synthetic distribution based on a theoretical model.
% }
% {
We explore the possibility of differentiating between these spin-down scenarios by combining recent stellar spin models with observations. We can then produce synthetic stellar distributions of the parameters sensitive to the spin-down mechanisms.
% }
% {
The theoretical model predicts a strong effect of the presence of an APSW on the relation between the disk truncation radius and the corotation radius, $\mathcal{R} = R_\mathrm{t}/R_\mathrm{co}$.
When comparing distributions of the ME and APSW scenarios, we find that a minimum number of $N_\mathrm{crit}\gtrsim 200$~stars is required to distinguish between the spin-down mechanisms on a high confidence level. 
Thanks to a novel observational technique, the parameter $\mathcal{R}$ can be derived in larger numbers than previously possible, allowing detailed tests of our model in the course of future observational campaigns.
% }
% {
% Being sensitive to the presence of an APSW, the parameter $\mathcal{R}$ is vital for distinguishing between the spin-down scenarios. Furthermore, the large-scale observation of $\mathcal{R}$ can provide insights into the stellar magnetic field strength distributions.
}



\keywords{      accretion, accretion disks --
                stars: protostars --
                stars: rotation
               }

\maketitle



==> resources/old_sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}


%  What is unclear?
The slow rotation of many T Tauri stars (with ages $\lesssim 10$~Myr and masses $\lesssim 2~\mathrm{M_\odot}$) is an unsolved problem.
The addition of angular momentum (AM) from an accreting circumstellar disk, plus contraction of the pre-main sequence star, should lead to spin-up \citep[e.g.,][]{Rebull2002}.  But multiple surveys of star-forming regions and young clusters show the distribution of rotation periods to be little changed over the 1--10 Myr lifetime of protoplanetary disks \citep[PPD, e.g.,][]{Rebull2006, Cody2010, Venuti2017, Rebull2020, Serna2021, Smith2023}. Most stars have rotation periods between 1 and 10 days, with a modal value of $\sim$3-4 days.  It is only after PPD dissipation that stars show the expected spin-up during their evolution toward the main sequence \citep[e.g.,][]{Gallet13}.

% It is only after  coinciding with the lifetimes of most protoplanetary disks \citep[PPDs, e.g.,][]{Pfalzner2024}.

% There are two spin-down mechanisms
The interaction between the star and the PPD is assumed to remove AM from the star, preventing the spin-up \citep[e.g.,][]{Koenigl91}.
Current stellar spin evolution models \citep[e.g.,][]{Gallet19, Pantolmos20, Ireland21, Ireland2022} explain the loss of AM by two mechanisms. First, magnetospheric ejections \citep[ME, ][]{Zanni13} are the result of the interaction from the relative motion of the stellar magnetic field through the partially ionized accretion disk, generating a toroidal magnetic field.  The resulting additional magnetic pressure can start a cycle of inflation, reconnection, and contraction of field lines.  During this cycle, some disk material is loaded onto stellar field lines creating a torque.  The second mechanism is accretion-powered stellar winds (APSW), where a fraction $W$ of the material accreted onto the star is ejected along open stellar magnetic field lines, removing AM \citep[e.g.,][]{Matt05APSW, Matt08, Matt12, Finnley18}.  The contribution of each mechanism is unclear since parameters such as $W$ are unknown and different mechanisms can produce the same rotation period distributions.


% We want to differentiate based on observed quantities
Here we use the spin evolution model of \cite{Ireland2022} to identify differences in the observable properties of T Tauri stars due to an APSW.  We construct a spin population model to estimate the minimum sample size of an observed distribution to differentiate between the no-wind ($W=0$ and only ME spin down the star) and wind ($W>0$) scenarios. 


==> resources/old_sections/results.tex <==
\section{Results}
\label{sec:results}



We assess the potential for statistical distributions of the SPM's key parameters, $P_\star$, $\Mdot$, and $\mathcal{R}$, to differentiate between the no-wind ($W = 0\%$) and wind ($W > 0\%$) scenarios.  As described in \sref{sec:pop_mod}, we generate and compare mock distributions of the SPM parameters to estimate the sample size required to achieve a $3\sigma$ level of statistical confidence.  We also include the expected observational uncertainties for our key parameters, increasing the scatter in the distributions.  The measurement of $\Dot{M}_\star$ is prone to uncertainties up to 0.35~dex \citep[e.g.,][]{Alcala2017, Manara22}.  
Stellar rotation periods can be observed with uncertainties of only a few percent \citep[e.g.,][]{Bowler2023}.  Thus, the uncertainty in $\mathcal{R}$ depends largely on the uncertainty in $R_\mathrm{t}$, which we take to be $\sim 0.2 R_\star$ (Venuti et al., in prep.; see Sec.~\ref{sec:obs}).


One way to distinguish between the no-wind and wind scenarios is the slope of the population on the $\mathcal{R}-\Mdot$ plane (see \fig{fig:theo_age}).
This slope depends on $B_\star$ and $\Mdot$.  In the case of no APSW, the slope of the whole population should be positive.  When including an APSW, the slope should decrease especially for high accretion rates ($\gtrsim 10^{-8}~\Msolpyr$).  The different slopes are shown in \fig{fig:slope_hist}.  As expected, the slope in the case of an APSW is smaller compared to the no-wind scenario, even including the expected observational uncertainties. The histogram on the right shows the distribution of the parameter $\mathcal{R}$.  For the no-wind and wind scenarios, the maxima of the distributions are located at $\approx 0.8$ and $\approx 0.6$.  For different sample sizes (ranging between 10 and 1000 stars), we generate distributions for $W=0\%$ and $W=1\%$, calculate the respective slopes, and repeat this process 1000 times. The resulting mean values and $3\sigma$ ranges of the slopes vs. sample size are shown in Panel (a) of \fig{fig:KDE} for $\tau_\mathrm{age}=2$~Myr. To distinguish between the wind and no-wind scenarios on a high confidence ($3\sigma$) level, we require a sample size of $N_\mathrm{crit} \ge 242$ stars. For older stars ($\tau_\mathrm{age}=5$~Myr), $N_\mathrm{crit}$ reduces to 198. The similar dependence of $\mathcal{R}$ (see \fig{fig:theo_age}) but smaller uncertainties (see \sref{sec:uncert}) are responsible for this lower value of $N_\mathrm{crit}$ for older stars.



\begin{figure}
    \centering
         \resizebox{\hsize}{!}{\includegraphics{assets/slope_hist.pdf}}
    \caption{
    Distribution of the SPM on the $\mathcal{R}-\Mdot$ plane for the wind and no-wind scenarios.
    The solid lines are the fitted slopes.
    The histograms of the parameter $\mathcal{R}$ are shown on the right.
    The stellar age is $\tau_\mathrm{age}=2$~Myr and each distribution contains 300 stars.
    }
    \label{fig:slope_hist}
\end{figure}




Alternatively, distinguish between the scenarios by comparing the overall parameter distributions, e.g., using a kernel density estimator (KDE), an estimate of the probability density function\footnote{We note that other authors have used the Kolmogorov–Smirnov (KS) test to quantify the similarity of different distributions \citep[e.g.,][]{Alexander2023}
The KS test, however, suffers from the limitation that its sensitivity decreases toward the tails of the distributions \citep[e.g.,][]{Lanzante2021}.}.  For comparing two distributions of the SPM parameters $P_\star$, $\Dot{M}_\star$, and $\mathcal{R}$, the respective KDEs are multiplied and the result is integrated over the whole parameter space.  The larger the value of this integral, the more the KDEs overlap, and the more similar the distributions are.   As a reference, we use a population with 1000~stars and assume $W=0\%$.  Similar to the previous method, this comparison is repeated 1000 times for different sample sizes assuming $W=0\%$ and $W=1\%$.  The normed result of the integral is shown in Panel (b) of \fig{fig:KDE}.  For this method, we find $N_\mathrm{crit}=365$.  Similarly to the comparison of the slopes, $N_\mathrm{crit}$ decreases to 302 for $\tau_\mathrm{age}=5$~Myr.  
The current disadvantage of this method is the theoretical reference model, which is based on a fixed $W$ value.
There are not sufficient measurements to compare the theoretical models to an observed distribution (see \sref{sec:obs}).
Once this changes, however, this method can provide a valuable comparison on a three-dimensional parameter space between observed and model distributions.






\begin{figure}
    \centering
         \resizebox{\hsize}{!}{\includegraphics{assets/KDEnew.pdf}}
    \caption{
    Statistical differentiation between the no-wind and wind scenarios.
    The slopes on the $\mathcal{R}-\Mdot$ plane and the normed value of the KDE overlap are shown in Panel (a) and (b).
    The solid lines are the mean values of the integrated KDE products after 1000 realizations of the SPM.  The shaded areas indicate the $3\sigma$ range.
    The stellar age is 2~Myr.
    The vertical dashed lines show the values of $N_\mathrm{crit}$.
    }
    \label{fig:KDE}
\end{figure}



==> resources/old_sections/spin_model.tex <==
\section{Spin population model}
\label{sec:spin_model}



\subsection{Stellar spin model}


We use the model outlined in \cite{Ireland2022}, in which the external torque acting on a star consists of two components, $\Gamma_\mathrm{ext} = \Gamma_\mathrm{SDI} +  \Gamma_\mathrm{W}$, with the star-disk interaction torque, $\Gamma_\mathrm{SDI}$ and the torque due to an APSW, $\Gamma_\mathrm{W}$. 
AM can be transferred between the star and disk via the accretion of disk material and magnetic star-disk interaction (ME). Accreted material adds AM to the star, while the magnetic star-disk interaction adds or removes AM from the star, depending on the ratio of the truncation radius to the corotation radius $\mathcal{R} = R_\mathrm{t}/R_\mathrm{co}$.  The corotation radius is given by $R_\mathrm{co} = (G M_\star / \Omega_\star^2)^{1/3}$, with the gravitational constant, $G$, the stellar mass, $M_\star$, and the stellar rotation rate, $\Omega_\star$.  The truncation radius, $R_\mathrm{t}$, is where the stellar magnetic forces disrupt the disk structure.  Following \cite{Ireland2022}, we use the expression
\begin{equation}\label{eq:Rt}
    R_\mathrm{t}/R_\star = \mathrm{min}\left( K_\mathrm{t,1} \Upsilon^{m_\mathrm{1}},~K_\mathrm{t,2} \Upsilon^{m_\mathrm{2}} f^{m_\mathrm{3}} \right)\, ,
\end{equation}
with the disk magnetization parameter, $\Upsilon = B_\star^2 R_\star^2 / (4 \pi \Dot{M}_\star v_\mathrm{esc})$, the fraction of the break up speed, $f$, and the constants $K_\mathrm{t,1}= 0.772$, $K_\mathrm{t,2}= 1.36$, $m_\mathrm{1}= 0.311$, $m_\mathrm{2}= 0.0597$, and $m_\mathrm{3}= -0.261$.  The stellar radius, magnetic field, and accretion rate are denoted as $R_\star$, $B_\star$, and $\Dot{M}_\star$, and $v_\mathrm{esc}$ is the stellar escape velocity $\sqrt{2GM_\star/R_\star}$. 

\citet{Ireland2022} divide the star-disk interaction torque $\Gamma_\mathrm{SDI}$ into three states:  In State 1, for $\mathcal{R}< 0.433$, accretion and MEs spin up the star.  For values of $0.433 \leq \mathcal{R} \leq 1.0$, accretion still spins up the star but MEs can exert a spin-down torque (State 2).  In State 3, for $\mathcal{R}> 1.0$, the spin-up torque due to accretion is negligible and the MEs spin down the star.  The expressions for the corresponding torques are:
%
\begin{equation}\label{eq:torque}
    \Gamma_\mathrm{SDI} = 
    \begin{cases}
    K_\mathrm{SDI,1} \Dot{M}_\star (G M_\star R_\mathrm{t})^{0.5} & \text{State~1} \\
    K_\mathrm{SDI,1} \Dot{M}_\star (G M_\star R_\mathrm{t})^{0.5}- K_\mathrm{SDI,2} B_\star^2 R_\star^6/R_\mathrm{co}^3 & \text{State~2} \\
    -K_\mathrm{SDI,2} B_\star^2 R_\star^6/R_\mathrm{t}^3 & \text{State~3} \\
    \end{cases}
\end{equation}
%
with the constants $K_\mathrm{SDI,1}= 0.909$ and $K_\mathrm{SDI,2}= 0.0171$.
The torque due to an accretion-powered wind, $\Gamma_{W}$, can be written as $\Gamma_\mathrm{W} = - \Dot{M}_\mathrm{W} \Omega_\star R_\mathrm{A}^2$ \citep[e.g.,][]{Ireland2022} with the mass loss rate $\Dot{M}_\mathrm{W} = W \Mdot$ and $R_\mathrm{A}$ is the Alfvén radius.
The parameter $W$ defines the mass-loss rate of the APSW and ranges at $W\lesssim 2\%$ \citep[][]{Browning16, Pantolmos20}.
We note that $W$ does not account for the complete ejection ratio of the inner star-disk interaction region that can reach up to $\sim 60\%$ and include multiple processes such as APSW, MEs, or MHD winds \citep[e.g.,][]{Watson2016, Serna2024}.

This study compares two wind scenarios; $W=0\%$, corresponding to no APSW, and $W=1\%$.  One key parameter of the spin model is the fraction $\mathcal{R}$ \citep[e.g.,][]{Gallet19, Pantolmos20, Ireland21, Ireland2022}.  For a given star ($M_\star$ and $R_\star$ known), $\Omega_\star = 2\pi/P_\star$ sets $R_{\rm co}$, while $R_{\rm t}$ depends on $\Dot{M}_\star$ and $B_\star$.  Furthermore, the value of $\mathcal{R}$ is a measure of the rotational state of the star, for increasing values of $\mathcal{R}$, the spin-up (spin-down) tendency decreases (increases).  Thus, $P_\star$, $\Dot{M}_\star$, and $\mathcal{R}$ define the torque components and rotational properties of a given star.

\subsection{Equilibrium state}\label{sec:equi_theo}

As described in \cite{Ireland2022} and \cite{Mueller2024}, the dependence of $\Gamma_{\rm SDI}$ on rotation is stabilizing and can cause a star to evolve toward an equilibrium, or zero-torque, rotational state within a timescale $ \tau_\mathrm{AM} = J_\star / \Gamma_\mathrm{ext} \lesssim 1-2$~Myr, with $J_\star$ the stellar angular momentum.  An extra, positive external torque causes the star to spin up, the corotation radius to contract, $\mathcal{R}$ to increase, and $\Gamma_{\rm SDI}$ to decrease.  Conversely, a negative external torque will cause $\Gamma_{\rm SDI}$ to increase. 
This behavior is illustrated in \fig{fig:schem_plot}.   Increasing $\mathcal{R}$, which corresponds to faster rotation periods, causes the net torque to decrease, causing the star to spin down, $R_{\rm co}$ to increase, and stabilizing $\mathcal{R}$ and $P_\star$.
Because an APSW removes AM from the star, the equilibrium state is reached at lower values of $\mathcal{R}$ and higher values of $P_\star$.
The effect of the changing moment of inertia of the contracting star can be neglected since the contraction is slow compared to $\tau_\mathrm{AM}$ for the stellar masses and ages studied in this work \citep[e.g.,][]{Ireland2022}.



\begin{figure}
    \centering
         \resizebox{\hsize}{!}{\includegraphics{assets/schem_plot.pdf}}
    \caption{
    Net torque in units of the stellar angular momentum vs $\mathcal{R}$ and $P_\star$ for two values of the wind parameter $W$.  The stellar parameters are as follows: $M_\star = 0.5~\mathrm{M_\odot}$, $B_\star = 0.5$~kG, $\Mdot = 3\times10^{-9}~\Msolpyr$, and $\tau_\mathrm{age}=2$~Myr.
    The zero-torque condition is indicated as the horizontal dashed line.
    }
    \label{fig:schem_plot}
\end{figure}

The equilibrium state for the no-wind scenario with $W=0\%$ and the wind scenario $W=1\%$ is shown in \fig{fig:theo_age} over a range of stellar accretion rates typical for T Tauri stars and two different values of $B_\star$.
We consider stellar ages of $\tau_\mathrm{age} = 2~\mathrm{Myr}$ (solid lines) and $\tau_\mathrm{age} = 5~\mathrm{Myr}$ (dashed lines).  For comparison, we added the observed range of stellar accretion rates for stellar ages ranging from 1~Myr to 8~Myr \citep[cyan and yellow lines, from][]{Betti2023}.
For the range of observed accretion rates of $\Mdot\lesssim 10^{-8}~\Msolpyr$, the influence of an APSW on the value of $\mathcal{R}$ is considerable.  For higher accretion rates, the effect of the APSW is larger and the difference between the no-wind and wind scenarios is more distinct.  On the other hand, higher values of $B_\star$ strengthen the MEs and the relative effect of the APSW decreases.  The mass dependence of the equilibrium state is small compared to the effect of an APSW.



The equilibrium state shown in  Fig.~\ref{fig:theo_age} is based on fixed stellar and disk parameters.  However, the parameters do not stay constant but evolve over Myr.  For example, the stellar radius contracts during pre-main sequence evolution, and the accretion rate decreases during the Class II phase.  As a result, the equilibrium value of $\mathcal{R}$ changes over time.
These long-term evolutionary changes of the stellar parameters, however, do not result in a significant deviation from the equilibrium state once the star reaches it \citep[e.g.,][]{Ireland2022, Mueller2024}.  In addition to the long-term changes in stellar parameters, short-term variations can affect the stellar spin more severely (see Sec.~\ref{sec:uncert}).








\begin{figure}
    \centering
         \resizebox{\hsize}{!}{\includegraphics{assets/theo_age2.pdf}}
    \caption{
    Equilibrium state values of $R_\mathrm{t}/R_\mathrm{co}$ over stellar accretion rates.
    We compare the no-wind (blue lines) with the wind (red lines) scenario for two stellar ages, $\tau_\mathrm{age}=2~\mathrm{Myr}$ and $\tau_\mathrm{age}=5~\mathrm{Myr}$.
    Magnetic field strengths of 0.1~kG (Panel a) and 1.0~kG (Panel b) are shown.
    For comparison, the observed range of stellar accretion rates is shown for stellar ages between 1~Myr and 8~Myr (cyan and yellow lines).
    The stellar mass is $0.7~\mathrm{M_\odot}$.
    }
    \label{fig:theo_age}
\end{figure}


\subsection{Effect of short-term variability}\label{sec:uncert}


Some stellar properties also exhibit short-term variability (timescales of $\tau_\mathrm{var} \lesssim$~years), especially $\Mdot$ \citep[e.g.,][]{Manara22} and $B_\star$ \citep[e.g.,][]{Johnstone14, Reiners22}.  As a result, a star in its equilibrium state is subjected to a variation in its parameters and can experience a spin-up or spin-down torque.
Typical literature values for these variations are 0.40~dex for $\Dot{M}_\star$ \citep[e.g.,][]{Manara22} and 0.48~dex for $B_\star$ \citep[e.g.,][]{Johnstone14, Reiners22}.


Based on these variations, we calculate the torque that acts on a star when $\Mdot$ and $B_\star$ deviate from their equilibrium values.  
In \fig{fig:delta}, the respective torques are shown over a range of (equilibrium) stellar magnetic field strengths for 2~Myr old stars.  
Starting from the equilibrium values, we randomly vary $\Mdot$ and $B_\star$ within the variation range and calculate the torques on the star assuming that it still rotates at the equilibrium rate ($\tau_\mathrm{var} \ll \tau_\mathrm{AM}$).  
This process is repeated 1000 times and the solid and dashed lines mark the $1\sigma$ range.  Spin-up (spin-down) torques, $\Delta_\mathrm{spin~up}$ ($\Delta_\mathrm{spin~down}$), are marked as solid (dashed) lines.  The values are similar for the no-wind and wind scenarios.  When increasing the stellar age to 5~Myr, the values of $\Delta_\mathrm{spin~up}$ and $\Delta_\mathrm{spin~down}$ decrease by a factor of $\approx 2/3$ due to the smaller stellar radii for older stars and the resulting smaller torques \citep[see \equo{eq:torque} and, e.g.,][]{Serna2024}.  Since these variations are unpredictable, we assume a star may deviate randomly from its equilibrium state within $2\Delta_\mathrm{spin~up}$ and $2\Delta_\mathrm{spin~down}$.



\begin{figure}
    \centering
         \resizebox{\hsize}{!}{\includegraphics{assets/delta_final2.pdf}}
    \caption{
    % Torques due to the variations of the parameters in units of the stellar angular momentum, $\tau_\mathrm{AM}^{-1}$, over a range of equilibrium magnetic field strengths.
    % The spin-up (down) torques are shown in solid (dashed) lines.  The stellar age is 2~Myr.
    Effect of a short-term deviation from the equilibrium state (as described in \sref{sec:uncert}).
    The resulting torques that act on the star, in units of the stellar angular momentum, $\tau_\mathrm{AM}^{-1}$, are shown over a range of equilibrium magnetic field strengths.
    The spin-up (down) torques are shown in solid (dashed) lines.  
    The stellar age is 2~Myr.
    }
    \label{fig:delta}
\end{figure}








\subsection{Schematics of the stellar population model (SPM)}\label{sec:pop_mod}


In this section, we describe the main assumptions of the SPM, which can be summarized as follows: 1) Most stars with ages $\tau_\mathrm{age} \gtrsim 1-2$~Myr have reached their equilibrium state. 2) In their equilibrium state, there is a significant difference in the value of $\mathcal{R}$ when comparing the no-wind and wind scenarios (see \fig{fig:theo_age}).  3) Due to variations in stellar parameters, stars can deviate from their equilibrium state within $2\Delta_\mathrm{spin~up}$ and $2\Delta_\mathrm{spin~down}$.


Based on these assumptions, we generate a population of stars in three steps. 
%First step: Mstar, Rstar, and Bstar
First, we select a stellar mass according to the initial mass function presented in \cite{Chabrier2014} between 0.2 and 1.0~$\mathrm{M_\odot}$.  The stellar radius is chosen based on the isochrones of \cite{Baraffe15} for a selected age.
% Second step: Mdot including observational uncertainty
In the second step, the accretion rate is chosen based on the relations presented in \cite{Betti2023}, allowing a scatter of two standard deviations.  Specifically, for $\tau_\mathrm{age}=2$~Myr, we use $\log\Dot{M}_\star = 2.12 \log M_\star -8.11$ and for $\tau_\mathrm{age}=5$~Myr, $\log\Dot{M}_\star = 2.43 \log M_\star -8.21$.  The $1~\sigma$ dispersion is 0.76~dex and 1.06~dex.
% Step 3: calculate the stellar spin for a random value of Bstar and check is delta is fullfilled
In the third step, we randomly choose a magnetic field strength from a uniform distribution between 0.1 and 2.0~kG\footnote{We note that this assumes that the variability in $B_\star$ and $\Mdot$ are uncorrelated.}.
For stellar rotation periods between 0.3 and 50~days \citep[observed range in, e.g.,][]{Smith2023} we calculate $R_\mathrm{t}$, $R_\mathrm{co}$, and $\Gamma_\mathrm{ext}$ \citep[according to][]{Ireland2022} and evaluate if $2\Delta_\mathrm{spin~down}\leq \tau_\mathrm{AM}^{-1} \leq 2\Delta_\mathrm{spin~up}$.  From all periods that fulfill this torque balance condition, we randomly choose the star's rotation period.
We discuss the sensitivity of our results on the choice of these distributions in \sref{sec:sens}.


Before showing the results of the SPM, we highlight the importance of the parameter $\mathcal{R}$ for distinguishing between the no-wind and wind scenarios. The equilibrium state and the torques due to variations in the stellar parameters, strongly depend on the magnetic field strength.
For a given accretion rate and rotation period, the value $\mathcal{R}$ gives an estimate of the magnitude of $B_\star$ independent of $W$ (see \equo{eq:Rt}).
Without a measurement of $\mathcal{R}$ and only $\Mdot$ and $P_\star$ available, the values of $\mathcal{R}$ and $B_\star$ are degenerate (covariant), preventing quantitative determinations.




